Evaluating the Gamma-Ray Evidence for Self-Annihilating Dark Matter from the Virgo Cluster

Based on three years of Fermi Large Area Telescope (LAT) gamma-ray data of the Virgo cluster, evidence for an extended emission associated with dark matter pair annihilation in the b b-bar channel has been reported by Han et al. [1]. After an in depth spatial and temporal analysis, we argue that the tentative evidence for a gamma-ray excess from the Virgo cluster is mainly due to the appearance of a population of previously unresolved gamma-ray point sources in the region of interest. These point sources are not part of the LAT second source catalogue (2FGL), but are found to be above the standard detection significance threshold when three or more years of LAT data is included.

==> PaxHeader/virgo.tex <==
18 gid=1187464677
17 uid=971529787
20 ctime=1343299419
20 atime=1343299421
38 LIBARCHIVE.creationtime=1343285134
24 SCHILY.dev=234881026
23 SCHILY.ino=41291328
18 SCHILY.nlink=1

